SCAR: Power Side-Channel Analysis at RTL-Level

Power side-channel attacks exploit the dynamic power consumption of cryptographic operations to leak sensitive information of encryption hardware. Therefore, it is necessary to conduct power side-channel analysis for assessing the susceptibility of cryptographic systems and mitigating potential risks. Existing power side-channel analysis primarily focuses on post-silicon implementations, which are inflexible in addressing design flaws, leading to costly and time-consuming post-fabrication design re-spins. Hence, pre-silicon power side-channel analysis is required for early detection of vulnerabilities to improve design robustness. In this paper, we introduce SCAR, a novel pre-silicon power side-channel analysis framework based on Graph Neural Networks (GNN). SCAR converts register-transfer level (RTL) designs of encryption hardware into control-data flow graphs and use that to detect the design modules susceptible to side-channel leakage. Furthermore, we incorporate a deep learning-based explainer in SCAR to generate quantifiable and human-accessible explanation of our detection and localization decisions. We have also developed a fortification component as a part of SCAR that uses large-language models (LLM) to automatically generate and insert additional design code at the localized zone to shore up the side-channel leakage. When evaluated on popular encryption algorithms like AES, RSA, and PRESENT, and postquantum cryptography algorithms like Saber and CRYSTALS-Kyber, SCAR, achieves up to 94.49% localization accuracy, 100% precision, and 90.48% recall. Additionally, through explainability analysis, SCAR reduces features for GNN model training by 57% while maintaining comparable accuracy. We believe that SCAR will transform the security-critical hardware design cycle, resulting in faster design closure at a reduced design cost.

==> Sections/Related.tex <==
\section{Related Work} \label{sec:related}

Existing research has developed a technique known as PSG-TG, that focuses on power analysis is performed on hardware designs to identify potential power side-channel leakage \cite{zhang2021psc}. It involves examining the power consumption patterns during the execution of the design using test pattern generation. RTL-PSC achieves automated power side-channel leakage assessment by extracting the RTL representation, generating a power model, performing power analysis, and identifying vulnerabilities, enabling efficient evaluation of power side-channel leakage at the register-transfer level \cite{he2019rtl}. 

% Researchers have also focused on analyzing power and noise signals in integrated circuits at the layout level to identify potential side-channel leakage points \cite{lin2020fast}.

% By leveraging efficient simulation techniques, the methodology enables thorough assessment of power-noise side-channel vulnerabilities in integrated circuit designs. Modeling and simulating power consumption of integrated circuit chips to identify potential side-channel leakage was proposed by \cite{tsukioka2019fast}. 

